Few-shot Fine-grained Image Classification via Multi-Frequency Neighborhood and Double-cross Modulation

Traditional fine-grained image classification typically relies on large-scale training samples with annotated ground-truth. However, some sub-categories have few available samples in real-world applications, and current few-shot models still have difficulty in distinguishing subtle differences among fine-grained categories. To solve this challenge, we propose a novel few-shot fine-grained image classification network (FicNet) using multi-frequency neighborhood (MFN) and double-cross modulation (DCM). MFN focuses on both spatial domain and frequency domain to capture multi-frequency structural representations, which reduces the influence of appearance and background changes to the intra-class distance. DCM consists of bi-crisscross component and double 3D cross-attention component. It modulates the representations by considering global context information and inter-class relationship respectively, which enables the support and query samples respond to the same parts and accurately identify the subtle inter-class differences. The comprehensive experiments on three fine-grained benchmark datasets for two few-shot tasks verify that FicNet has excellent performance compared to the state-of-the-art methods. Especially, the experiments on two datasets, "Caltech-UCSD Birds" and "Stanford Cars", can obtain classification accuracy 93.17\% and 95.36\%, respectively. They are even higher than that the general fine-grained image classification methods can achieve.

==> figures-pdf/fg8.tex <==

\begin{tikzpicture}
\matrix [row sep = 0.05cm,column sep= 0.05cm,nodes= { inner xsep = 11.5px,inner ysep = 18.5px,align = center,font=\fontsize{9}{6}\selectfont}]{
\node[fill = {rgb,255:red,96;green,74;blue,123}] {65.73};&
\node[fill = {rgb,255:red,128;green,100;blue,162}] {65.61}; &
\node[fill = {rgb,255:red,128;green,100;blue,162}] {65.36};& 
\node[fill = {rgb,255:red,128;green,100;blue,162}] {65.29}; & 
\node[fill = {rgb,255:red,204;green,193;blue,218}] {64.45};\\
\node[fill = {rgb,255:red,179;green,162;blue,199}] {64.72};&
\node[fill = {rgb,255:red,128;green,100;blue,162}] {65.42}; &
\node[fill = {rgb,255:red,128;green,100;blue,162}] {64.82};&
\node[fill = {rgb,255:red,204;green,193;blue,218}] {64.50}; &
\node[fill = {rgb,255:red,204;green,193;blue,218}] {64.33};\\
\node[fill= {rgb,255:red,128;green,100;blue,162}]{65.69};&\
\node[fill = {rgb,255:red,204;green,193;blue,218}] {64.47}; &\
\node [fill = {rgb,255:red,128;green,100;blue,162}]{64.81};& 
\node[fill = {rgb,255:red,128;green,100;blue,162}] {64.99}; & 
\node[fill = {rgb,255:red,230;green,224;blue,236}] {64.14};\\
\node [fill = {rgb,255:red,204;green,193;blue,218}]{65.09};&
\node [fill = {rgb,255:red,204;green,193;blue,218}]{64.47}; &
\node[fill = {rgb,255:red,204;green,193;blue,218}] {64.61};&
\node[fill = {rgb,255:red,230;green,224;blue,236}] {64.10}; &
\node[fill = {rgb,255:red,230;green,224;blue,236}] {63.80};\\
\node[fill = {rgb,255:red,230;green,224;blue,236}] {64.19};&
\node [fill = {rgb,255:red,230;green,224;blue,236}]{65.09}; &
\node [fill = {rgb,255:red,230;green,224;blue,236}]{63.84};&
\node[fill = {rgb,255:red,230;green,224;blue,236}] {63.81}; & 
\node [fill = {rgb,255:red,230;green,224;blue,236}]{63.73};\\
};
\end{tikzpicture}


